Challenging Environments for Traffic Sign Detection: Reliability Assessment under Inclement Conditions

State-of-the-art algorithms successfully localize and recognize traffic signs over existing datasets, which are limited in terms of challenging condition type and severity. Therefore, it is not possible to estimate the performance of traffic sign detection algorithms under overlooked challenging conditions. Another shortcoming of existing datasets is the limited utilization of temporal information and the unavailability of consecutive frames and annotations. To overcome these shortcomings, we generated the CURE-TSD video dataset and hosted the first IEEE Video and Image Processing (VIP) Cup within the IEEE Signal Processing Society. In this paper, we provide a detailed description of the CURE-TSD dataset, analyze the characteristics of the top performing algorithms, and provide a performance benchmark. Moreover, we investigate the robustness of the benchmarked algorithms with respect to sign size, challenge type and severity. Benchmarked algorithms are based on state-of-the-art and custom convolutional neural networks that achieved a precision of 0.55 and a recall of 0.32, F0.5 score of 0.48 and F2 score of 0.35. Experimental results show that benchmarked algorithms are highly sensitive to tested challenging conditions, which result in an average performance drop of 0.17 in terms of precision and a performance drop of 0.28 in recall under severe conditions. The dataset is publicly available at https://github.com/olivesgatech/CURE-TSD.

==> challenge_details.tex <==

\begin{itemize}[leftmargin=*]

\item \textbf{Decolorization} tests the contribution of color information, which was implemented using \texttt{Black \& White} Color Correction filter version $1.0$. The filter settings were: \texttt{Reds}$=40$, \texttt{Yellows}$=60$, \texttt{Greens}$=40$, \texttt{Cyans}$=60$, \texttt{Blues}$=20$, and \texttt{Magentas}$=80$. We utilized multiple adjustment layers to compound the effect of the color correction filter and created multiple distinct levels of this challenge.

\item \textbf{Lens Blur} tests the effect of image details, which was implemented using \texttt{Camera Lens Blur} filter version $1.0$. The filter settings were: \texttt{Blur radius} was set to $2, 4, 6, 8,$ and $10$ for levels $1-5$ and \texttt{Iris Shape} was Hexagan, everything else was set as default.

\item \textbf{Codec Error} tests the effect of encoder/decoder error, which was implemented using \texttt{Time Displacement} filter version $1.6$. The filter settings were: \texttt{Max Displacement Time} was set to $0.1, 0.2, 0.3, 0.4,$ and $0.5$ for levels $1-5$, everything else was set as default.

\item \textbf{Darkening} tests the effect of image contrast and overall brightness, which was implemented using \texttt{Exposure} filter version $1.0$. The filter was set to modify the master channel \texttt{Exposure} parameter to be $-1, -3, -5, -7,$ and $-9$ for levels $1-5$, everything else was set as default.

\item \textbf{Dirty Lens} tests the effect of dust and dirt on the camera lens through occlusion, which was implemented using a set of dusty and smudged lens images superimposed on the video.

\item \textbf{Exposure} tests the effect of malfunctioning exposure control in acquisition, which was implemented using \texttt{Exposure} filter version $1.0$. The filter was set to modify the master channel \texttt{Exposure} parameter to be $1$, $3$, $5$, $7$, and $9$ for levels $1-5$, everything else was set as default.

\item \textbf{Gaussian Blur} tests the effect of image details, which was implemented using \texttt{Gaussian Blur} filter version $3.0$. The filter settings were: \texttt{Bluriness} was $5, 10, 15, 20,$ and $25$ for levels $1-5$, everything else was set as default. Unlike \textbf{Lens Blur}, \textbf{Gaussian Blur} is equally distributed in all directions, which leads to less structured blurred objects.

\item \textbf{Sensor Noise} tests the effect of acquisition noise, which was implemented using \texttt{Noise} filter version $2.6$. The filter settings were: \texttt{Amount of Noise} parameter was set to $20, 40, 60, 70,$ and $71$ using $5$ adjustment layers that were compounded to generate levels $1-5$, everything else was set as default.

\item \textbf{Rain} tests the effect of occlusion due to rain, which was implemented using \texttt{Gradient Ramp} generator version $3.2$ with colors \texttt{\# 0F1E2D} and \texttt{\# 5A7492} to create a blueish hue over the video, and \texttt{CC Rainfall} generator from Cycore Effects HD 1.8.2 version $1.1$. The setting of \texttt{CC Rainfall} generator were: \texttt{Drops} was set to $10000, 20000, 50000,$ and $100000$ and \texttt{Opacity} was $25\%$ using $5$ adjustment layers that were compounded to generates levels $1-5$, everything else was set as default.

\item \textbf{Shadow} tests the effect of non-uniform lighting due to shadow, which was implemented using \texttt{Venetian Blinds} filter version $2.3$. The filter settings were: \texttt{Transition Completeness} was $47\%$, \texttt{Dirrection} was $0x+0.0^{\circ}$, \texttt{Width} was $142$, and \texttt{Opacity} was $15\%, 30\%, 45\%, 60\%$, and $75\%$ for levels $1-5$, everything else was set as default.

\item \textbf{Snow} tests the effect of occlusion due to snow, which was implemented using \texttt{Glow} filter version $2.6$ with color \texttt{\# FFFFF} to create a white hue over the video, and \texttt{CC Snowfall} generator from Cycore Effects HD 1.8.2 version $1.1$. The setting of \texttt{Glow} filter were: \texttt{Glow Threshold} was $55\%$, \texttt{Glow Intensity} was $1.4$, \texttt{Glow Operation} was Screen, and \texttt{Glow Dimension} was Horizontal. The setting of \texttt{CC Snowfall} generator were: \texttt{Drops} $10000, 50000, 100000$, and $140000$ using $9$ adjustment layers that were compounded to generates levels $1-5$, everything else was set as default.  

\item \textbf{Haze} tests the effect of occlusion due to haze, which was implemented using \texttt{Ellipse Shape Layer} filter version $1.0$ with radial gradient fill using color \texttt{\# D6D6D6} in the center with $100\%$ opacity and color \texttt{\# 000000} with $0\%$ opacity on the edges, \texttt{Smart Blur} version $1.0$, \texttt{Exposure} version $1.0$, and \texttt{Brightness \& contrast} version $1.0$. The shape and focal point location of the \texttt{Ellipse} was manually controlled to closely follow the furthest point in the video, which created a sense of depth to the scene and emulated the behaviour of haze in realistic settings. The setting of \texttt{Smart Blur} filter were: \texttt{Radius} was $3$, and \texttt{Threshold} was $25$. The setting of \texttt{Exposure} filter for the master channel were: \texttt{Radius} was $-1$, and \texttt{Gamma Correction} was $1$. The setting of \texttt{Brightness \& Contrast} filter were: \texttt{Brightness} was $-34$, and \texttt{contrast} was $-13$. Additionally, we utilized \texttt{Solid Layer}, which was created from color \texttt{\# CECECE} and opacity $10\%, 20\%, 30\%, 40\%$, and $50\%$ to add difficulty to levels $1-5$.

\end{itemize}


==> fig_scenes.tex <==
\begin{figure*}[tbp!]
\centering
\begin{minipage}[b]{0.23\linewidth}
  \centering
\includegraphics[trim=0cm 0cm 0cm 0cm,width=\linewidth]{./Figs/scenes/fig_1b}
  \vspace{0.15cm}
  \centerline{\footnotesize{(a) exposure }}%\medskip
\end{minipage}
\begin{minipage}[b]{0.23\linewidth}
  \centering
\includegraphics[trim=0cm 0cm 0cm 0cm,width=\linewidth]{./Figs/scenes/fig_1c}
  \vspace{0.15cm}
  \centerline{\footnotesize{(b) snow }}%\medskip
\end{minipage}
\begin{minipage}[b]{0.23\linewidth}
  \centering
\includegraphics[trim=0cm .0cm 0cm 0cm,width=\linewidth]{./Figs/scenes/fig_1d}
  \vspace{0.15cm}
  \centerline{\footnotesize{(c) haze }}%\medskip
\end{minipage}
\begin{minipage}[b]{0.23\linewidth}
  \centering
\includegraphics[trim=0cm 0cm 0cm 0cm,width=\linewidth]{./Figs/scenes/fig_1e}
  \vspace{0.15cm}
  \centerline{\footnotesize{(d) rain }}%\medskip
\end{minipage}
\begin{minipage}[b]{0.23\linewidth}
  \centering
\includegraphics[trim=0cm 0cm 0cm 0cm,width=\linewidth]{./Figs/scenes/fig_1f}
  \vspace{0.15cm}
  \centerline{\footnotesize{(e) dirty lens  }}%\medskip
\end{minipage}
\begin{minipage}[b]{0.23\linewidth}
  \centering
\includegraphics[trim=0cm 0cm 0cm 0cm,width=\linewidth]{./Figs/scenes/fig_1g}
  \vspace{0.15cm}
  \centerline{\footnotesize{(f) noise }}%\medskip
\end{minipage}
\begin{minipage}[b]{0.23\linewidth}
  \centering
\includegraphics[trim=0cm 0cm 0cm 0cm,width=\linewidth]{./Figs/scenes/fig_1h}
  \vspace{0.15cm}
  \centerline{\footnotesize{(e) rain }}%\medskip
\end{minipage}
\begin{minipage}[b]{0.23\linewidth}
  \centering
\includegraphics[trim=0cm 0cm 0cm 0cm,width=\linewidth]{./Figs/scenes/fig_1i}
  \vspace{0.15cm}
  \centerline{\footnotesize{(f) decolorization }}%\medskip
\end{minipage}
\vspace{-0.2cm}
\caption{Challenging scene examples from the CURE-TSD dataset.}
\label{fig:scenes}
\vspace{-0.5cm}
\end{figure*}
